Interpretable Sequence Classification via Discrete Optimization

Sequence classification is the task of predicting a class label given a sequence of observations. In many applications such as healthcare monitoring or intrusion detection, early classification is crucial to prompt intervention. In this work, we learn sequence classifiers that favour early classification from an evolving observation trace. While many state-of-the-art sequence classifiers are neural networks, and in particular LSTMs, our classifiers take the form of finite state automata and are learned via discrete optimization. Our automata-based classifiers are interpretable---supporting explanation, counterfactual reasoning, and human-in-the-loop modification---and have strong empirical performance. Experiments over a suite of goal recognition and behaviour classification datasets show our learned automata-based classifiers to have comparable test performance to LSTM-based classifiers, with the added advantage of being interpretable.

==> Makefile <==
PREFIX  = main
TEXFILE = $(PREFIX).tex
PSFILE  = $(PREFIX).ps
PDFFILE = $(PREFIX).pdf

       
all:	dolatex \
	dobibtex \
	dolatex2

dolatex:
	pdflatex $(TEXFILE)

dolatex2:
	pdflatex $(TEXFILE)

dodvips:
	dvips -t letter -Ppdf -G0 -j0 -o$(PSFILE) $(PREFIX)

dopdf:
	ps2pdf $(PSFILE)

do2up:
	psnup -2 $(PSFILE) $(PREFIX)_2.ps

do4up:
	psnup -4 $(PSFILE) $(PREFIX)_4.ps

dobibtex:
	bibtex $(PREFIX)

clean:
	rm  *dvi *log *aux *bbl *blg


==> sections/computation.tex <==

\subsection*{The Observer's Planning Task\eat{? Plan Generation? Computation?}\eat{Computing Solutions to the\\ Active Goal Recognition Problem}}\label{comp}

% In this section, we realize a computational solution to the APR problem, relative to its specification in the previous section.

% In this section, we discuss how the observer may utilize its agency to eliminate hypotheses. To do so, we first formalize means by which to test hypotheses.


As discussed, the observer is assumed to have a goal of its own such as aiding or impeding goal achievement. We refer to this goal as $G_O$. Thus, given an active goal recognition problem, the observer must decide how to best act in order to \eat{gather additional information and} generate observations, facilitate early recognition and achieve $G_O$.
\eat{\textit{eliminate} hypotheses in $\optimalhyps$ as early as possible and achieve $G_O$.} The task of deciding how to act is then one of planning - devising a course of action to reach $G_O$.


\begin{definition}
Given an active goal recognition problem $\activeGRtuple$ and the observer's goal $G_O$, the observer's planning task is $\langle \fluents, \actions, \sensingactions, \init', G_O \rangle$ where $\Sigma_O = \langle \fluents, \actions, \sensingactions \rangle$, and $\init'$ is the logical filtering of $O$ wrt the belief state $b$ for $\init_O$, following \citeauthor{amir2003logical} (\citeyear{amir2003logical}).


% \commentms{elaborate on filtering? just say that we compile away observations by progressing wrt action and effect? - from PO-PRP ``Prog(s, a, e) is the progression of s wrt a’s effect e and is defined as usual for planning with conditional effects (Reiter 2001)" }. 
% \commentms{`wrt $\init_O$' maybe needs to be a belief state}
% , and $\statecons$ is a logical formula representing additional state constraints that must be enforced throughout the plan.
\end{definition} 

If $O$ comprised only actions, with no observed properties of state, we would simply progress $b$ wrt to the actions in $O$. Logical filtering instead progresses $b$ wrt actions and \textit{filters} $b$ wrt to properties of state by eliminating every state $s \in b$ which is inconsistent with the observation.
%
While the observer may in some settings be restricted to sensing the world, in other settings it may be able to affect the state of the world, the actor's goal or plan, or even the set of hypotheses. 
%
For example, the observer may introduce an obstacle along some path and test the actor's next action which, in the altered domain, will make clear the actor's goal\eat{(similarly to the \textit{offline} goal recognition design setting \cite{keren2014goal})}.
%
Further, the observer's actions may be prohibited from affecting $\hyps$ at all or in undesirable ways (e.g., the observer could dispose of all the pasta in the kitchen, thus eliminating the pasta making goal from $\hyps$). Finally, obfuscation, privacy, and safety constraints may be enforced when the observer does not wish for its actions to be observable by the actor or for its goal to be inferred, or when we wish to prohibit the observer from endangering itself or the actor.

We assume that the actor's goal ($G^*$) does not change and formally discuss how to preclude the observer's world-altering actions from rendering possible hypotheses impossible and vice versa. To this end, we say that \textit{achievable($\Sigma$,$G$)} holds in some belief state $b$ \textit{iff} there exists a belief state $b'$ where $G$ $\in$ $\hyps$ holds that is reachable from the belief state $b$ with the action theory $\Sigma$.
%
Let $\tau$ be a solution to the planning task $\langle \fluents, \actions, \sensingactions, \init', G_O \rangle$, let $b$ be the belief state for $\init'$, and let $b''$ be a belief state that may result from executions (partial or full) advised by $\tau$ and that does not immediately follow the execution of a sensing action in $\tau$.
%
We say that an observer is \textit{non-intervening} \textit{iff} \{\textit{achievable($\Sigma_A$,$G$)} $\mid$ \textit{achievable($\Sigma_A$,$G$)} holds in $b$\} and
\{\textit{$\lnot$achievable($\Sigma_A$,$G$)} $\mid$ \textit{$\lnot$achievable($\Sigma_A$,$G$)} holds in $b$\} (both interpreted as conjunctive formulae) hold in $b''$.


\subsection*{Testing Hypotheses} 
We are interested in solutions to the observer's planning task $\obsPlanTask$ comprising \textit{tests} which are performed in the world by the observer and whose outcomes eliminate hypotheses in $\mathcal{G}$. Following \citeauthor{mcilraith1992tests} (\citeyear{mcilraith1992tests}):



\begin{definition} \label{simpleTest} A \textbf{simple test} is a tuple $\langle IC, \omega\rangle$ where $IC$, the initial conditions for the test, is a conjunction of literals and $\omega \in \Omega$ is a sensing action.

% \commentms{maybe we only need the def for a test for hyp space. also maybe change $s$ to $a$}

 \end{definition}

% In our example, $\langle$ \textit{connected-to(host1),check-root-access-log} $\rangle$ is an example of such a test. A test could be to sense what \act does next or sense the world. 




% \begin{definition}
% \label{testForHypSpace} A test $\langle IC, s\rangle$ is a test for a set of hypotheses $\mathcal{G}$ iff $s$ is executable in $I \cup \statecons$.
% \end{definition}


% \begin{definition} \label{discTest} 
% A discriminating test is
%  \end{definition}
 
% \begin{definition} \label{relevantTest} 
% A relevant test is
% \end{definition}
 
%  \commentms{maybe minimal test def here}
 
% \begin{definition} [Minimal Test \cite{mcilraith1992tests}] \label{minTest}  A test for the hypothesis space $\mathcal{G}$
% is minimal iff... \eat{iff for no proper subconjunct $IC'$ of $IC$ is $(IC',s)$ a test which can produce identical test outcomes as $(IC,s)$ for $\mathcal{G}$.\textbf{VERIFY}}
% \end{definition}

% In other words, minimal tests do not require unnecessary initial conditions and only include those conditions which are required for producing the test outcome. 

Tests may also be \textit{complex}, comprising a series of simple tests interleaved with world altering actions whose execution satisfies the initial conditions necessary to perform the various simple tests \cite{mcilraith1992tests}. Tests can be encoded as \textit{complex actions} \cite{mci-fad-nmr02f} which enable the planner to achieve a subtask without search. More generally, planning with macro-actions (e.g., \cite{fikes1972learning,korf1987planning}) can potentially improve the efficiency of plan generation by exploiting reusable subplans and reducing plan length.

% exploit reusable subplans, thereby potentially improving planning efficiency and generating shorter plans. More generally, planning with macro-actions 

% \commentms{Planning with some form of macro-actions (e.g., (Fikes, Hart, \& Nilsson 1972; Sacerdoti 1974; Korf 1987; McIlraith \& Fadel 2002; Erol, Hendler, \& Nau 1994)) can dramatically improve the efficiency of plan generation. The advantage of using macro-actions in general, are two fold. By encapsulating programs into operators plan length is reduced, which in turn significantly reduces the search space. Also, operators provide a means of achieving a subtask without search. This leads to increased performance of planners - from ``On planning with programs that sense"}

% and possibly eliminate the hypotheses.


% .\commentms{The observer’s planning task then consists
%  of selecting appropriate tests (relative to $G_O$), and planning to satisfy.. , and possibly subsequent actions comprising a reaction to the test outcomes (e.g., planning to assist or hinder the actor, made easier or possible with a smaller hypothesis set which resulted from the test's outcome due to ** newly eliminated hypotheses** hypothesis elimination )} %Appropriate tests are selected based on 
% % In this work, we are interested in synthesizing such complex tests for the purposes of hypothesis elimination in service of APR. 


\begin{definition}[Test Outcome]
The outcome of a simple test $\langle IC, \omega\rangle$ is $\textsc{Obs}(\omega)$.
% one of $obs(a)$,$\lnot obs(a)$.
\end{definition}

% A test outcome, $\alpha$, can either \textit{refute} or \textit{confirm} hypotheses in $\mathcal{G}$.


% pect some states (i.e., only some test outcomes). I.e., if we sense both coffee and tea, then this is fine because it confirms both hypotheses. We require that a relevant test either discriminates between hyps or not discriminate and confirm. That is also the goal. Maybe penalize not discriminating so that planner prefers discrimination? A complex test could be, for example, an SPR process where ACT is queried. It could also be a series of world altering and sensing actions executed by OBS and that do not involve interaction with ACT. We will explore the latter type of test in the next section. \textbf{or maybe don't restrict to this type of test since we can theoretically handle both types - perhaps only talk about this above where we define the DPR task and say it subsumes SPR (instead of only queries, we have general tests)}\\ 


% \commentms{Φ, is a logical formula representing additional state constraints that must be enforced throughout the plan; and}\\

% In the PR context, we say that a test outcome $\alpha$ \textbf{refutes} a hypothesis $G \in \mathcal{G}$ \textit{iff} the hypothesis is no longer achievable from $I \cup \alpha$ if $h$ is a goal and executable from $I \cup \alpha$ if the hypothesis is a plan. We also informally say that a test outcome $\alpha$ \textbf{confirms} a hypothesis $h \in H$ \textit{iff} $\alpha$ explains $h$. In the next section, we will present algorithms which solve the APR problem based on a concrete definition of hypothesis confirmation.

% Next, we discuss how hypotheses may be eliminated via \textbf{refutation} and \textbf{confirmation}. 




% \commentms{maybe define test outcome - i.e., $p$ or $\lnot p$} In the next section, we will discuss a number of approaches to test generation for APR which will formally define confirmation and refutation criteria of hypotheses. 

\begin{definition}[Refutation]\label{refutation}
A test outcome $\testoutcome$ refutes a hypothesis $G \in \hyps$ iff there does not exist a belief state $b'$ where $G$ holds that is reachable (with $\Sigma_A$) from the logical filtering of $\testoutcome$ with $b$ for $\init'$.\eat{\commentms{Filtering may cause $b'$ to be empty which is fine since if we get an empty belief set as the result of the filtering, the goal is not reachable from an empty belief set and thus the hyp is refuted}}\eat{\commentms{we have to assume no false beliefs - only uncertainty, otherwise the definition doesn't work. Epistemics.... The observer asks: ``given my view of the world ($\init'$) and the new information that I have acquired ($\testoutcome$), can the actor achieve $G$?" It does not ask whether actor can still be \textit{intending} $G$ since it assumes that actor does not have false beliefs and therefore knows that $G^*$ is possible. Further, If observer already knows some $\phi$ then it won't test for it!}}
% \commentms{can we use $\{\testoutcome\} \cup \init$}


% iff $G$ is not achievable from $\{\testoutcome\} \cup \init$.\commentms{there does not exists a sequence of actions that, when applied to $\{\testoutcome\} \cup \init$ (this may have to be the progression of $\init$ with $\testoutcome$, $G$ holds as a result (in the belief state?)}\commentms{}
\end{definition}

% \commentms{Maybe add to def: if the hypothesis is a plan (sequence of actions from $\mathcal{A}$) then $\testoutcome$ refutes the hypothesis \textit{iff} the plan is not executable from $\testoutcome \cup \mathcal{I}$}\\

For example, if $G$ is \textit{cooked(pasta)} and the observer discovers that there is no pasta in the kitchen, then $G$ can be refuted since acquiring pasta is not part of the actor's action theory and having pasta is necessary to achieve $G$. Future work will address a setting where the actor may harbor \textit{false beliefs} and may, for example, falsely believe there is pasta in the cabinet and thus devise a plan for an unachievable goal. An assistive agent could proactively offer to fetch some pasta from the store.

% if $G$ $=$ \textit{bought(privateIsland)} and the observer discovers that the actor does not have sufficient funds to achieve $G$, we may refute $G$. Alternatively, 

% may hold false beliefs such  ..}Further, while we assume that the actor does not have false beliefs, one can imagine how the actor may falsely believe there is pasta in the cabinet and therefore plan to cook it, while not knowing that the goal is not achievable. An assistive agent could discover that there is no pasta and offer to go and fetch some from the store.

% In the intervening active PR setting, the observer could also refute certain hypotheses by, for example, disposing of

% both roads that lead to the bank are closed, then under \act's restricted action set (planning domain) we can refute $h$. We assume that \act does not have false beliefs.

% restricted resource which makes a plan unachievable (e.g., time, money,…)
% * Something is physically impossible under restricted action set (no pasta in cabinet - you can’t go and buy it because it’s not in your action set)




\begin{definition}[Confirmation]\label{confirmation}
A test outcome $\testoutcome$ confirms a hypothesis $G \in \mathcal{G}$ iff there exists a sequence of world-altering actions $\pi = a_1,\ldots,a_n$, $\pi \in \Pi^{*}(G)$, and some prefix $a_1,\ldots,a_m$ of $\pi$, $1 \leq m \leq n$, such that $\testoutcome$ holds in $b'$ which is the result of performing $a_1,\ldots,a_m$ in $b$ for $\mathcal{I}_A$.

% \commentms{if we want to be more general then we can talk about the set of optimal policies - If the test outcome is part (a path) of any execution advised by a policy in the set of optimal policies then...}
% A test outcome $\testoutcome$ confirms a hypothesis $G \in \mathcal{G}$ iff $\testoutcome$ is on an optimal path (policy?) to $G$.
\end{definition}


% \commentms{maybe instead say that $\testoutcome$ confirms iff it EXPLAINS or CHARACTERIZES $h$ and say that we'll explain later. although this is general enough perhaps to fit both landmarks and LTL. LTL formula that is leanred is also on optimal path. we can also define \textbf{`weak confirmation'} where the test outcome is on a path that is almost optimal (defined by some bound on sub-optimality)}



A refuting or confirming test outcome can eliminate a hypothesis depending on the criteria by which a hypothesis space is defined. \citeauthor{mcilraith1992tests} (\citeyear{mcilraith1992tests}) define two types of hypothesis spaces with the following properties:

% , a \textit{consistency-based hypothesis space}, and an \textit{abductive hypothesis space}.

% \begin{definition} \label{CBHypSpace} A consistency-based hypothesis space is..
%  \end{definition}
 
% From \cite{mcilraith1992tests}:
\begin{pro}\label{elim_consis}
If $\hyps$ is a consistency-based hypothesis space, a test outcome $\testoutcome$ eliminates all hypotheses $G \in \hyps$ that are refuted by $\testoutcome$.
\end{pro}

% \begin{definition} \label{abdHypSpace} An abductive hypothesis space is..
%  \end{definition}

% From \cite{mcilraith1992tests}:
\begin{pro}\label{elim_abduc}
If $\hyps$ is an abductive hypothesis space, a test outcome $\testoutcome$ eliminates all
hypotheses $G \in \mathcal{G}$ that are not confirmed by $\testoutcome$. 
\end{pro}


% \textbf{In justification of optimality- say that they're expected to follow optimal given their perspective of the state of the world}

It follows that abductive hypotheses are eliminated by both refuting and non-confirming test outcomes. Our definition of confirmation (and thus of elimination) presupposes a 
%
% In the goal recognition setting, this definition of elimination via non-confirmation presupposes a
%
perfectly rational agent that follows optimal paths to the goal (relative to the observer's assumptions pertaining to the actor's model of the world). Indeed, this assumption (or slightly relaxed variations which tolerate paths that are `more or less' optimal) is either implicitly or explicitly made in most previous work on cost-based goal and plan recognition (e.g., \cite{ramirez2010probabilistic,sohrabi2016plan})\eat{, as well as our definition of elimination by lack of confirmation,}. While in some settings it is reasonable (or, in the absence of information about the actor, unavoidable) to assume optimality on behalf of the actor (e.g., a robot following a strict protocol can be assumed to (be attempting to) follow optimal plans), this assumption proves too strong in other instances and may cause the recognizer's performance to suffer\eat{ \cite{masters2019goal}}. \citeauthor{masters2019goal} (\citeyear{masters2019goal}) have identified that deviation from (expected) optimality may be caused by the actor's `irrationality', stemming from a number of possible reasons including a deceptive actor and the observer's misconceptions regarding the actor's model of the world.
%
% either a possibly different cost model, actual irrationality, or deceptive behavior.
%
The authors enable a recognition system to dynamically adapt to perceived irrationality (e.g., by lowering the confidence of its predictions) and as part of future work their approach can complement our definitions of elimination.
%
Finally, we note that test outcomes may be used by an active observer both to eliminate hypotheses and as additional evidence by which to weight hypotheses in a probabilistic setting.





% \begin{algorithm}[h!]
% \floatname{algorithm}{Algorithm 1:}
% \renewcommand{\thealgorithm}{}
% \caption{maybe caption}
% \label{fig:algorithm_APR}
% \begin{algorithmic}[1]
% \begin{small}
% \REQUIRE An active online PR problem $\langle \Sigma, I, \hyps, O \eat{\Omega}\rangle$
% %\linebreak
% \ENSURE $\hyps' \subseteq \hyps$
% \WHILE{\textit{\textsc{isAvailable}($o_{t+1} \in O$)}}
%     \STATE $\hyps'$ = \textsc{PRAlgorithm($O,\hyps$)}
%     \WHILE{\textbf{not} (\textsc{CheckEndingCriteria}($\hyps$) \\\textbf{or} \textit{\textsc{isAvailable}($o_{t+2} \in O$)} \textbf{or} \textit{timeout})}
%         \STATE  $\Pi$ = \textsc{GenerateTest($\hyps'$)} \commentms{OR generatePlan(...)}
%         \STATE \textit{testOutcome} = \textsc{ExecuteTest($\Pi$)} \commentms{OR executePlan(...)}
%         \STATE \textsc{UpdateObservations($O$, \textit{testOutcome})}\\ 
%         \STATE $\hyps'$ = \textsc{PRAlgorithm($O,\hyps$)}
%     \ENDWHILE{}
% \ENDWHILE{}

% \STATE RETURN $\hyps'$


% \end{small}

% \end{algorithmic}
% \label{alg1}
% \end{algorithm} 

% \subsection{Test Generation}
% \textbf{is this section needed?}
% Let $\hyps = \{G_1,G_2\}$. Assuming that following Line 2 of Algorithm 1, $\hyps' = \{G_1,G_2\}$ and given that the ending criterion is $|\hyps| = 1$, in Line 4 we wish to generate a test to either eliminate $G_1$ and not $G_2$ or eliminate $G_2$ and not $G_1$. To eliminate a hypothesis $h$ we may have to perform a sequence of world-altering actions in order to meet the initial conditions (the test setup) of the test that can refute or not confirm $G_i$. To generate such a sequence of actions, we leverage AI planning by translating the `elimination goal' into a goal that can be given to an off-the-shelf automated planner. In what follows we describe various approaches to `translate' the elimination goal to a planning goal. To ease exposition we assume that the ending criterion is $|\hyps| = 1$ and that the hypotheses are equally likely. In Section \ref{discussion} (or end of this one) we discuss different strategies which determine what hypotheses to focus on (i.e., try to eliminate).  

% to generate tests for hypothesis elimination. To this end, we describe a number of approaches to automatically specify a planning goal. 




\subsection*{Landmark-based Hypothesis Elimination}
% Hypothesis elimination can be done in different ways. For example, SPR queries ACT and subsequently refines the hypothesis space to reflect the test outcome (ACT's reply to the query). Sometimes, we do not wish to interrupt ACT and so...\\
% \textbf{Example:} In our example, one way to know that ACT's goal is not to make rice, but rather pasta is by looking in the cabinet and discovering that there is only pasta there (assume ACT knows the contents of the cabinet (we'll get to the case where we relax this assumption - maybe future work)). Formally, the outcome of the test of sensing the contents of the cabinet refutes RICE, leaving PASTA the only possible hypothesis.\commentms{note that the pasta may be on the counter, and so the landmarks is that pasta is in the cabinet AND not on counter (or vice versa)}\\\\

% In Line 3 of Algorithm 1 the observer must decide how to act in service of the recognition process. Recall that we derive the observer's planning task $\mathcal{P} = \obsPlanTask$ from an active goal recognition problem $\activeGRtuple$.

In what follows we discuss how to construct the observer's planning task. We assume that $\init_A$ defines a complete initial state and that $\sensingactions$ $=$ $\emptyset$ in $\Sigma_A$. Finally, to ease exposition, we assume that the observer's goal is to \textit{maximally eliminate} hypotheses in $\hyps'$ $\subseteq$ $\hyps$.
%
We focus on eliminating hypotheses by way of not confirming them and leverage \textit{fact landmarks} to do so. Following Hoffmann et al. (\citeyear{hoffmann2004ordered}):
% , more generally, the observer's goal could be to focus on specific hypotheses that are of interest to the observer (and its goal).
%
% Finally, to ease exposition, we assume that the observer's goal is to eliminate all hypotheses in $\hyps'$ but one. More generally, the observer's goal could be to maximally eliminate hypotheses in $\hyps'$ or to focus on specific hypotheses that are of interest to the observer (and its goal).
%
% \eat{\commentms{Maybe say this in terrorist example}}\eat{Thus, the observer must generate a plan to to eliminate all hypotheses but one. }We augment $\fluents$ with a special predicate \textit{eliminated($G_i$)} for each $G_i \in \hyps'$ and can then express $G_O$ as $(\eliminatedHyp{G_1} \land \ldots \land eliminated(G_{n-1})) \lor (eliminated(G_2) \land \ldots \land eliminated(G_n)) \lor \ldots$ (i.e., a disjunction of all combinations of $\optimalhyps$ of size $|\hyps'| - 1$).
%
%
%
% \citeauthor{hoffmann2004ordered}
% which capture \eat{the actions that must be taken or }properties that must hold in the world in order for some goal $G \in \hyps$ to be achieved. We \eat{focus on fact landmarks and }follow 

% \commentms{is to maximally eliminate hypotheses in $\hyps$. We thus augment $\fluents$ with the predicate \textit{eliminated($G_i$)} for every $G_i \in \hyps$. We further define a function which keeps track of the number of eliminated hypotheses}

%
% ground the elimination definitions from the previous section in 
% augment $\sensingactions$ with actions that encapsulate tests that can potentially eliminate hypotheses. To generate these tests we 
%
% One approach to hypothesis elimination via test generation and execution is landmark-based. 
%
% Landmarks for a certain goal $G \in \hyps$ capture the actions that must be taken or properties that must hold in the world in order for the goal to be achieved.
%

% That is, a what does it `look like' for an agent to achieve a certain goal, such as stealing data from a server? In the case of data theft, root access must be obtained before the data is stolen. 
% \commentms{(and syntactically restricted) - maybe talk about LTL - Behavior patterns can be obtained in a variety of ways. In this section we consider landmarks } 



% \commentms{There are many approaches to analyzing planning domains etc.}

% \textit{in(pasta,cabinet)} is an example of a \textit{landmark} for the goal PASTA. Formally:
% \textbf{Frame landmarks as patterns of behavior (syntactically restricted LTL formulae)}

\begin{definition}[Fact Landmark]
Given a classical planning task $\mathcal{P}$ $=$ $\PPOStuple$, a formula $l$ is a fact landmark in $\mathcal{P}$ iff $l$ is
true at some point along all plans that solve $\mathcal{P}$. \eat{A landmark is a type of formula (e.g., a conjunctive or disjunctive formula) over a set of facts that must be satisfied at some point along all valid plan executions.}
\end{definition}

% In our example, achieving the goal \textit{(data-stolen host1} requires gaining root access to \textit{host1}. Thus, one of the landmarks in $\mathcal{L}$ is \textit{(root-access-obtained host1)}. 

We do not consider disjunctive landmarks. Let $\LMGoal$ be the set of landmarks for some goal $G \in \hyps$ given an action theory and an initial state.  
%
%
% We say that a landmark $l$ $\in$ $\LMGoal$ is \textit{protected} \textit{iff} there does not exist a belief state $b'$ where $G$ holds that is reachable (with $\Sigma_A$) from the logical filtering of $\lnot l$ with $b$ from $\init'$.
%
% \eat{We say that a landmark $l$ $\in$ $\LMGoal$ is \textit{protected}\commentms{state protected}\eat{ or fragile or unchangable or protected or irrevocable or unachievable or crucial} \textit{iff} $l$ must be true prior to the execution of any valid plan that solves $\mathcal{P}$.}
% We say that a landmark $l$ $\in$ $\LMGoal$ is \textit{protected} \textit{iff} it must hold throughout the execution of any valid plan that solves $\mathcal{P}$.
%
% \commentms{We simplify for now but a more interesting case is where the landmark must hold throughout the plan or until some point in the plan when another landmark $l' = \lnot l$ must hold. For example, \textit{coffee} must hold until a point in the plan when \textit{coffee} does not hold since it is used}
%
% there does not exist a belief state $b'$ that is reachable (with $\Sigma_A$) from the belief state $b$ of $\init_A$ such that $\lnot l$ holds in $b$ and $G$ holds in $b'$.
%
% \eat{$l$ is not achievable from $I$\commentms{need to define achievable in section 2 - maybe using belief state}.}
%
%
We assume that $\sensingactions$ (in $\Sigma_O$) is augmented with sensing actions $\omega \in \sensingactions$ that encapsulate simple tests $\langle IC, \omega'\rangle$, where $\textsc{Pre}(\omega)$ = $\textsc{Pre}(\omega') \land IC$ and $\textsc{Obs}(\omega)$ is the test outcome.\eat{ that allow the observer to sense observable fluents in $\fluents$.} \eat{\commentms{say that the tests are encoded as complex actions - see how it's done in McIlraith paper - not necessarily in $\sensingactions$. tests are assumed to be encoded as macro actions}The preconditions of each such sensing action $\omega$ are then the initial conditions of the test and . }Recalling Definition \ref{confirmation}:

% \begin{pro}\label{ref_LM}
% A test outcome $\testoutcome$ refutes a hypothesis $G \in \hyps$ if $\lnot\testoutcome$ is a protected landmark for $G$\eat{ and there does not exist a landmark $l' \in \LMGoal$ such that $$}.
% \end{pro}

\begin{pro}\label{conf_LM}
A test outcome $\testoutcome$ confirms a hypothesis $G \in \hyps$ if $\testoutcome$ is a landmark for $G$ (i.e., $\testoutcome \in \LMGoal$). 
\end{pro}

% Let $\testoutcome_1,...,\testoutcome_n$ be a set of test outcomes such that $\testoutcome_j$ is a protected landmark for $G_j \in \hyps$

Proposition \ref{conf_LM} follows from Definition \ref{confirmation} since if $\testoutcome$ is a landmark for $G$, it is made true at some point along all plans in $\Pi^{*}(G)$. Thus, there exists a prefix $a_1,\ldots,a_m$ of some plan in $\Pi^{*}(G)$ which satisfies $\testoutcome$.
Assuming $\hyps$ is abductively defined it follows from Propositions \ref{elim_abduc} and \ref{conf_LM} that:

% if a test outcome $\testoutcome$ is a unique landmark for $G_i \in \hyps$, it \textit{eliminates} all hypotheses $G_j \in \hyps$ such that $i \neq j$.

% and assuming $\hyps$ is ave these props inline}
% \begin{pro}\label{unach_elim_pro}
% A test outcome $\testoutcome$ eliminates a hypothesis $G \in \hyps$ if $\lnot\testoutcome$ is a protected landmark for $G$.

% % A test outcome $\testoutcome$ eliminates 
% % Let $\testoutcome_1,...,\testoutcome_n$ be test outcomes such that   protected landmarks for all $G_j \in \hyps$ where $i \neq j$, they eliminate all hypotheses but $G_i$. 
% \end{pro}

% % % Let $\testoutcome_1,...,\testoutcome_n$ be test outcomes where $\testoutcome_j$ is a protected landmark for $G_j \in \hyps$ where $i \neq j$, they eliminate all hypotheses but $G_i$. 

\begin{pro}\label{uniq_elim_pro}
If a test outcome $\testoutcome$ is a landmark for $G_i \in \hyps$ but not for $G_j \in \hyps$ (i.e., $\testoutcome \in \mathcal{L}_{G_i}$ and $\testoutcome \not\in \mathcal{L}_{G_j}$), then $\testoutcome$ \textit{eliminates} $G_j$.
\end{pro}

% we can now say that a test outcome $\testoutcome$ refutes a hypothesis $h \in H$ \textit{iff} $\lnot\testoutcome$ is a protected landmark for $h$. We further say that a test outcome $\testoutcome$ confirms a hypothesis $h \in H$ iff $\testoutcome$ is a landmark for $\testoutcome$.


% Thus, if $\testoutcome$ is a unique landmark (associated with some $G_i \in \hyps$), it only confirms $G_i$ and does not confirm any $G_j$ where $i \neq j$. 


% \commentms{ADD THIS if prop 6 is not clear - Since $\testoutcome$ only confirms $G_i$, all other hypotheses are not confirmed and thus eliminated. }



% \textbf{Planning-based Test Generation\quad}To ease exposition, we assume for the rest of the discussion that the ending criterion in Algorithm 1 is $|\hyps'| = 1$ and that all hypotheses in $\hyps$ are equally likely. To satisfy the ending criterion, we build on Propositions \ref{unach_elim_pro} and \ref{uniq_elim_pro} and generate tests to eliminate all hypotheses but one. To do so, we generate tests that attempt to either refute all hypotheses but one (Proposition \ref{unach_elim_pro}) or confirm one and only one hypothesis (Proposition \ref{uniq_elim_pro}). In what follows, we describe how to construct such tests automatically by casting the test generation task as a planning task.\commentms{describe the initial elements of the planning task $\Sigma$ taken from the PR problem in alg 1}
%
% whose solution is a test (or series of tests with world-altering actions in between) that can eliminate hypotheses.
%
% \textbf{Define contingent planning tuple in the landmark section - here's the tuple and $\mathcal{A}'$ is $\mathcal{A}$ + the augmented actions ans so on}
% To this end, we first 


\eat{\commentms{we maybe ONLY need most unique (uniqueness value) without defining a unique landmark - maybe just mentione that a unique landmark (i.e., landmark with a uniquness value of 1(???) eliminates all hyps but one}Similarly to \citeauthor{pereira2017landmark} (\citeyear{pereira2017landmark}), given a set of hypotheses $\hyps$, we say that a landmark $l$ is \textit{unique} \textit{iff}
%
% $|\{ G \in \hyps | l \in \LMGoal\}|$
%
$l \in \LMGoal$ for one and only one hypothesis $G \in \hyps$.}


% Then,
% the initial state of φ, Iφ, is updated with the given observations by advancing the state from the initial Iφ and applying
% all actions corresponding to the observations in Oφ

We apply the action observations in $O$ to $\init_A$ and extract (using $\Sigma_A$ and $\init_A$) the set $\LMHyps$ which comprises the sets of \eat{(**testable**)}landmarks\eat{ (that can be sensed by actions in $\sensingactions$)} ($\LMGoal$) for each hypothesis $G \in \hyps'$. From $\LMHyps$ we compute the set of landmarks $\LMGoalUnique$ with the highest \textit{`landmark uniqueness value'} which represents the information value of a given landmark (\citeauthor{pereira2017landmark} 2017, Equation 2). $\LMGoalUnique$ comprises the `most unique' landmarks such that each $l \in \LMGoalUnique$ belongs to a minimal number of $\LMGoal \in \LMHyps$\eat{\commentms{to be formal, we can USE min function}}. For example, a landmark $l \in \LMGoalUnique$ could be shared by two and only two hypotheses $G_1$ and $G_2$ and upon observing $l$, the observer can eliminate all hypotheses but $G_1$ and $G_2$ (following Proposition \ref{uniq_elim_pro}). 
%
% \commentms{maybe not - in the absence of unique landmarks... instead, if the highest uniqueness value is x, then...}, a landmark $l \in \LMGoalUnique$ could be shared
%
% From each set of landmarks in $\LMHyps$, we filter the \textit{achieved} landmarks based on the 
%
% For each observed action o in O, the algorithm computes all fact landmarks of G that are in the preconditions and effects of o in Line 7. As we deal with partial observations in a plan execution some executed actions may be missing from the observation sequence, thus whenever we identify a fact landmark, we also infer that its predecessors must have been achieved in Line 8.
%
%
We augment $\fluents$ with a special predicate \eliminatedHyp{$G_i$} for each $G_i \in \hyps'$ (which we use to keep track of eliminated hypotheses\eat{for elimination bookkeeping}) as well as the predicate \textit{done}.
%
We generate a set of actions $\actions''$ and for each landmark $l \in \LMGoalUnique$ we add an action $a$ to $\actions''$ where $\textsc{Pre}(a) = l$ and $\textsc{Eff}(a)$ is a conjunction of \textit{done} and every \eliminatedHyp{$G_i$} such that $G_i \in \hyps'$ is eliminated by $l$ (i.e., \{\eliminatedHyp{$G_i$} $\mid$ $l$ $\not\in$ $\mathcal{L}_{G_i}\}$).
%
\eat{ (i.e., all $G_j \in \hyps'$ such that $i \neq j$)}
%
\eat{Next, we generate a set of actions $\actions'''$ where for each hypothesis $G_i \in \hyps'$ and for each protected landmark $l \in \mathcal{L}_{G_i}$ we add an action $a$ to $\actions'''$ such that $\textsc{Pre}(a) = \lnot l$ and $\textsc{Eff}(a)$ is \eliminatedHyp{$G_i$}. We assume that all protected landmarks for $G \in \hyps'$ hold in $\init_A$ and $\init'$.}
%
\eat{The condition of the conditional effect of all actions $a \in \actions''$ is assumed to be trivially satisfied.}

% and compute the sets of unique landmarks and protected landmarks\eat{, $\LMGoalUnique$ and $\LMGoalUnachievable$, respectively\commentms{do we need these}}.

% Rather than generating the set of unique landmarks, we generate the set of landmarks with the highest landmark uniqueness value 


% Alternatively, if the observer is trying to maximally eliminate hypotheses, we can instead extract the set of landmarks with the highest \textit{`landmark uniqueness value'} which represents the information value of a given landmark \cite{pereira2017landmark}.\eat{We can similarly treat the protected landmarks\commentms{?}.}





% We generate a set of actions $\actions''$ where for each unique landmark $l\eat{ \in \LMGoal}$ we add an action $a$ to $\actions''$ where $\textsc{Pre}(a) = l$ and $\textsc{Eff}(a)$ is a conjunction of all \eliminatedHyp{$G_j$} such that $G_j \in \hyps'$ is eliminated by $l$ (i.e., all $G_j \in \hyps'$ such that $i \neq j$).

%
%$\text{\textit{eff(a)}} = \eliminatedHyp{G_i}$.
%
% $a \in \actions_{elimConfirm}$, $pre$
%
% augment $\mathcal{A}$ with (non-sensing) actions that correspond to each unique landmark $l \in \LMGoalUnique$ where the precondition of the action is $l$ and the effect is a conjunction of all \eliminatedHyp{$G_i$} where such that $G_i \in \hyps$ is eliminated by $l$.
%
% For each protected landmark $l \in \LMHyps$

% Depending on the recognition setting, we can use protected landmarks t

To ensure that the observer is non-intervening, as defined previously in this section,
%
% \commentms{FIX!}we set $\statecons$ to be a non-intervening constraint. We compile $\statecons$ into the planning task by 
%
we eliminate all actions $a$ $\in$ $\actions$ where \textsc{Eff($a$)} includes a landmark (or a negated landmark) $l$ $\in$ $\LMHyps$. While this method of enforcing non-intervention is maximally prohibitive to the observer, it is minimally disruptive to the actor. We will explore other, less prohibitive methods of enforcing non-intervention (e.g., Linear Temporal Logic \cite{pnueli1977temporal}) in future work.
%
% To compile $\statecons$ into the planning task and ensure the observer's actions do not make possible hypotheses impossible,
% %
% enforce the observer's non-intervention,
%
% we set $\statecons$ to be the conjunction of all protected landmarks $l \in \LMHyps$.\eat{ such that $l$ holds in $b$ for $\init'$ as well as the conjunction of all landmarks $l \in \LMGoal$, for every $G \in \hyps'$, such that $l$ must hold prior to the execution of any valid plan for $G$.}\eat{\commentms{- doesn't the set of protected LMs include these? No. every protected LM must hold prior to plan execution but not every LM that must hold prior to every plan is a protected LM (e.g., coffee in kitchen LM)}} We then add $\statecons$ to $G_O$ and to $\textsc{Pre}(a)$ for every $a \in \actions$, thus ensuring that $\statecons$ holds in any belief state that may result from partial or full executions of any solution to the planning task.
% To ensure the observer's actions do not make impossible hypotheses possible, we can keep track of protected landmarks that have been discovered, via sensing, to not hold (\eat{, by Proposition \ref{ref_LM},}thus refuting the corresponding hypothesis)\eat{ or using unsolvability analyses \cite{sreedharan2019can}} and preclude the observer's actions from making them hold. \eat{E.g., if there is no pasta in the kitchen (and the actor cannot acquire it), $\statecons$ should preclude the observer from fetching pasta from the store.}We leave formal treatment to future work. \eat{\citeauthor{pozanco2018counterplanning} (\citeyear{pozanco2018counterplanning}) formalize the notion of \textit{counterplanning landmarks} which the observer utilizes to impede goal achievement. These landmarks could be used to prevent the observer from affecting $\hyps$. Further,} 

% \citeauthor{pozanco2018counterplanning} (\citeyear{pozanco2018counterplanning}) discuss important considerations that arise as a consequence of the observer and actor executing their plans in a common environment and their formalization of mutex actions and joint execution can complement our work.

% While we do not treat the case where the 

% To ensure the observer's actions do not make impossible hypotheses possible, for every $G \in \hyps$ such that $G \not\in \hyps'$, we add the conjunction of negated protected landmarks in $\LMGoal$ (that hold in $\init_A$ and $\init'$) to $\statecons$. E.g., if there is no coffee in the kitchen (and the actor cannot acquire coffee)\eat{(i.e., a negated protected landmark for \textit{made(coffee)}}, $\statecons$ precludes the observer from fetching coffee from the store\eat{, making the goal possible}. We add $\statecons$ to $\textsc{Pre}(a)$ for every action $a \in \actions$ as well as the goal $G_O$, thus ensuring that $\statecons$ holds in any belief state that may result from partial or full executions of any solution to the planning task.

% (i.e., $G$ is not considered a possible hypothesis), 
% (e.g., the observer may fetch coffee from the store, making the \textit{made(coffee)} goal possible), 

% We do not enforce 


% \eat{We do not treat the condition where the observer's actions should not cause $G^*$ to change. \commentms{SAY WHY, REPHRASE,OR DON'T HAVE THIS CONDITION IN THE NON-INTERVENING DEF}} \commentms{To bar the observer from making a falsified hypothesis true, we can also add the conjunction of the negated protected landmarks to the preconditions of actions in $\actions$. that way, the observer's actions cannot, for instance, buy coffee just to make the coffee hypothesis possible.}

% (e.g., 
% axioms \cite{thiebaux2005defense} 

% We compile 
% This is akin to compiling away axioms 



\eat{Test outcomes may fail to eliminate hypotheses in $\hyps$.} \eat{We force the planner to exhaust all possible tests by adding a special action $a$ to $\actions$ where $\textsc{Pre}(a)$ is a conjunction of all protected landmarks and all negated unique landmarks.
%
% $\lnot \textsc{Pre}(a)$ for $a \in \actions''$ (all negated unique landmarks) and a conjunction of $\textsc{Pre}(a)$ (all protected landmarks) for $a \in \actions'''$  the negated unique landmarks and all protected landmarks that appear in the preconditions of the special actions with which $\mathcal{A}$ is augmented.
%
\eat{$\textsc{Pre}(a)$ only holds if all test outcomes failed to eliminate hypotheses in $\hyps'$.\eat{\commentms{what if we only elimnate some? what if goal is to maximally eliminate?}} $\textsc{Eff}(a) = \text{\textit{testsExhausted}}$.}}
% \commentms{if we need to be more formal: $\bigwedge_{i=1} \lnot{lu}_{i} \bigwedge \lnot{lmunachivable}_{i}$ (the conjunction of unachivables needs to be the conjunction of all preconditions of all the special elimination by refutation actions)}

% similarly to before with actions with the precondition being the conjunction of protected landmarks and the effect being \textit{refuted\_i} (corresponding to hypothesis $G_i$).
% \eat{To eliminate hypotheses via refutation, following Proposition \ref{unach_elim_pro}, we must observe a protected landmark for each hypothesis but one. }\eat{Next, for each hypothesis $G_i \in \hyps$, the `elimination' goal comprises one protected landmark for every $G_j$ where $i \neq j$ (if $G_j$ has more than one protected landmarks then we have a disjunction of all of them. }

% Then, the planning goal is \textit{eliminated} $\lor$ \textit{testsExhausted}. 
%\eat{ \cup \actions'''} \eat{ G_O \lor \textit{testsExhausted}$.}
\eat{In effect, we task the planner with *****either eliminating all hypotheses but one (either by confirming one hypothesis and not confirming all others or by refuting all hypotheses but one) or exhausting all tests.} 
%
The planning task is then $\mathcal{P}$ $=$ $\langle \fluents', \actions', \sensingactions, \init', G_O \rangle$, where $\actions' = \actions \cup \actions''$ and $G_O$ $=$ \textit{done}\eat{ $\land$ $\statecons$, and $\statecons$ is compiled into $\mathcal{P}$}.
$\mathcal{P}$ can then be given to a planner that generates a conditional plan $\tau$ that solves $\mathcal{P}$.\eat{where $G_O$ $\lor$ \textit{testsExhausted} holds in the resulting belief states.}\eat{***Note that $\tau$ may comprise a series of simple tests with world-altering actions in between (e.g., move to a different location or log on to a server) to satisfy the tests' initial conditions.\commentms{one test}***} As $\tau$ may include sensing actions, it may be the case that their outcomes will not eliminate any hypotheses and thus $G_O$ may not hold in some resulting belief states. In such a case, $\tau$ is considered a \textit{weak} plan that reaches the goal under at least one possible set of action outcomes of the actions in the plan, as opposed to a \textit{strong} plan which is a closed policy that achieves the goal in all resulting belief states \cite{cimatti2003weak}.
%
% wrt and is thus not guaranteed to reach the goal \commentms{ that . 
%
Notice also that to satisfy $G_O$ the planner need only include one action $a \in \actions''$ in $\tau$ but we may straightforwardly force it to exhaust all tests.\eat{ The planner can be forced to exhaust all tests by generating a series of simple tests with world-altering actions in between. This can be done in various ways including complex actions and a function that keeps track of the number of eliminated goals which the planner is forced to maximize.} 



\begin{thm}[Complexity]\label{thm:complexity}
Let $\mathcal{P} = \langle \fluents', \actions', \sensingactions', \init', G_O \rangle$ be the observer's planning task. If $\init'$ does not define a complete initial state and $\sensingactions' \neq \emptyset$ then $\mathcal{P}$ is a conditional planning problem and deciding whether there exists a solution for $\mathcal{P}$ is 2-EXPTIME-complete.
% The complexity of generating a plan in Line 4 of Algorithm 1 given a planning task $\langle \fluents', \actions', \sensingactions', \mathcal{I}_O, G_O', \statecons \rangle$ is 2-EXPTIME-complete.
\end{thm}
% \commentms{change to this phrasing: Given a diagnostic planning problem (ΣSD, Init, Φ, G), if I ∪Init∪Φ does not define a complete initial state and Ω 6= ∅ then this is a conditional planning problem and deciding whether there exists such a plan is 2-EXPTIME-complete.}

Theorem \ref{thm:complexity} follows from \citeauthor{rintanen2004complexity}'s results on the complexity of
conditional planning \cite{rintanen2004complexity}.

% execute the plan - because things constantly change in the world and we need to ‘hope’ that test we come up with is still relevant

% The planning goal is now a conjunction of all \textit{refuted\_i} with \textit{eliminated} $\lor$ \textit{testsExhausted}. Thus, after augmenting the action theory with actions corresponding to both unique and protected landmarks, the planner will generate an action tree that will either eliminate all hypotheses but one or exhaust all possible (landmark-based) tests to achieve this elimination objective. \commentms{how much action tree and conditional planning background do we need}

% we want either success with unique LMs or failure with unique LMs but success with refutation or failure with refutation. we don't care about order of tests - they're all gonna eliminate all but one! we just need to make sure that the all tests done predicate only becomes true if we've tried all refutation-based and confirmation-based.

% \textbf{Test Execution}
% In Line 5, we execute the action tree (policy) generated by the planner and note that the execution will terminate either with a positive test outcome or a negative one (for all tests). notice that the test is thus neither relevant nor discriminating since a possible test result neither confirms nor denies any hypothesis.



% reflects a positive test result (which eliminates all but one hypothesis) or  all tests conducted (including for refutation) and negative results from all OR a big disjunction of the positive results 



% The test that achieves this goal is a tree where one branch holds a test outcome where $\testoutcome$ is a unique landmark. That branch satisfies the elimination of all hypotheses but the one associated with the unique landmark $\testoutcome$. To the conjunctive goal we also add any protected landmarks associated with hypotheses which should be eliminated. 





% We thus translate the elimination goal (i.e., for $h \in H$ \textit{eliminated($h$)} except one of them) to knowing whether the unique landmark corresponding to the $h$ we don't want to eliminate

% We can formally define the refutation and confirmation o hypothesis given a test outcome:

% \begin{definition}[Refutation]
% A test outcome $\testoutcome$ refutes a hypothesis $h \in H$ iff $h$ is not achievable from $\testoutcome \cup I$.
% \end{definition}

% \begin{definition}[Confirmation]
% A test outcome $\testoutcome$ confirms a hypothesis $h \in H$ iff $\testoutcome$ is a landmark for $\testoutcome$.
% \end{definition}

% \textbf{Example} To illustrate our approach, we use the \textsc{Terrorist} domain proposed by \citeauthor{pozanco2018counterplanning} (\citeyear{pozanco2018counterplanning}), where a terrorist has committed an attack in the center of a city and is attempting to leave the city. The police (the observer) know that the terrorist (the actor) can leave the city by either $G_1$ (airport), $G_2$ (train station), or $G_3$ (bus terminal) and thus $\hyps = \{G_1,G_2,G_3\}$. The police wishes to prevent the terrorist from leaving the city by setting a control point along paths leading to $G_i \in \hyps$. However, the police can only set one control point and must therefore first perform goal recognition to infer the terrorist's goal. The police have control over cameras located in various locations around the city which provide the goal recognition algorithm with observations. However, assuming $O$ is empty (i.e., the terrorist hasn't been detected by any of the cameras) the goal recognition algorithm will deem all hypotheses equally likely, thus forcing the police to set the control point at a randomly selected location. 

% Now consider that the police has a drone at their disposal, which they can deploy to scan various locations in the city. We can now model the example as an active goal recognition problem, where the observer's goal is to eliminate hypotheses in order to prevent the actor from achieving its goal (in fact, the observer need not eliminate all hypotheses...). A unique landmark $l$ for $G_1$ is that the actor is at a certain point along the path from the city center to $L1$ (which is itself a landmark for $G_1$). Thus, one of the actions added to $\actions$ includes the precondition $l$ and the effect is $\eliminatedHyp{G_2} \land \eliminatedHyp{G_3}$. Thus, after the goal recognition algorithm in Line 3 returns $\hyps' = \optimalhyps = \{G_1,G_2,G_3\}$, in Line 4 a conditional plan $\tau$ is generated which advises the deployment of the drone to the location in $l$. Upon executing $\tau$, the drone may locate the terrorist and eliminate $G_1$ and $G_2$, and thus $\hyps' = \{G_1\}$. Note that $l$ may not be the first landmark to be tested in $\tau$ if no ordering is enforced between tests for the various landmarks. For example, one can exploit the ordering of the landmarks and prioritize testing for landmarks that are expected to be achieved first. \commentms{there's no need to eliminate all but one. It suffices to have eliminated (G2) or eliminated (G3 ) - we don't need both to set control}
% may not advise that $l$ be the first landmark to be tested. However, we can enforce an ordering between 


% let us consider a simple domain where a terrorist has committed an attack in the center of a city. Figure 2 shows the road network for this problem. The city police (α) knows that the terrorist (φ) wants to leave the city by either G1 (airport), G2 (train station), or G3 (bus terminal); so, Gφ = {G1, G2, G3}. The police has control over some cameras located at key points around the city (represented as nodes in Figure 2). The police actions consist of stopping the terrorist by setting a control at any of those points (Aα). So, the police wants to: (1) quickly know where the terrorist wants to go (G0φ); and (2) stop him/her as soon as possible to avoid panic breaking out. When the cameras observe that the terrorist is at L1 (O1 = a1 ∈ Aφ), the police guesses that his/her goal is to reach G1 (G0φ) by doing goal recognition. The police only has resources to set one control. It knows that the terrorist must pass through L1, L2 and L3 to reach the airport. Although these four spots are counterplanning landmarks LΠφ,Πα , the police can only set the control at L2, L3 and G1 before the terrorist reaches those places. Finally, the police goal Gα will be to set the control at L2 since it is the FCL; i.e. the first spot where the terrorist can be effectively stopped.

% \textbf{Let's assume that the police have drones in that the test includes the test setup which involves moving the drone to a certain area. Then, the test observes weather the terrorist is in the area or not}

% \textbf{May be necessary for terrorist example - We can enforce order of tests (as we do for observations) by forcing this test to be selected before that test\\
% Say that we can exploit the structure of the landmark graph and look for the earlier landmarks first.\\
% Say in experiments that in our simulations the set of hyps wa}


% We will use our example to illustrate one iteration of Algorithm 1. Initially, $\hyps = \{\text{\textit{(vandalized host1)}},
% \text{\textit{(data-stolen host1)}}\}$ and $O = \text{\textit{(access-obtained host1)}}$ and thus in Line 2 the PR algorithm cannot discriminate between the two hypotheses and returns $\hyps' = \hyps$. Since the ending criterion ($|\hyps'| = 1$) is not met, the algorithm proceeds to generate a test in Line 3. One unique landmark in the computed set is \textit{(root-access-obtained host1)}. The planner generates an action tree for \textit{eliminated $\lor$ testsExhausted} which comprises a sensing action $a$ with \textit{obs(a) = (root-access-obtained host)}. Assuming root access has been obtained by the attacker, in Line 5 the test outcome will be \textit{(root-access-obtained host)}. After $O$ is updated with the test outcome, the call to the PR algorithm in Line 7 will return $\hyps' = \{\text{\textit{(data-stolen host1)}}\}\}$ since the vandalism hypothesis is eliminated by the test outcome. 

% \textbf{INTRUSION DETECTION!!!}In our example, we have seen that the outcome of the test involving \textit{sense\_cabinet} was \textit{in(pasta,cabinet)} and also \textit{$\lnot$in(rice,cabinet)}. As discussed, one of the landmarks of PASTA is \textit{in(pasta,cabinet)} (and also not on counter, which we know). Thus, the outcome of the test confirms PASTA. More importantly, however, the test outcome \textit{refutes} RICE since one of its landmarks is \textit{(in(rice,cabinet) $\land$ $\lnot$on(rice,counter)) $\lor$ ($\lnot$in(rice,cabinet) $\land$ on(rice,counter))}. Since this cannot hold (FORMALIZE), the outcome (ALPHA!!) refutes RICE.\\



\subsection*{Computation}
% As we are operating in an online setting, we assume that the sequence of observations for an active goal recognition problem $\mathcal{P} = \activeGRtuple$ is generated by the observer, using the `previous' active goal recognition problem. If no such problem exists, we start with $\mathcal{P}$ where $O$ is empty. 

% Given $\mathcal{P}$, we construct and solve the observer's planning task from $\mathcal{P}$ as previously discussed in this section. Throughout the execution of $\tau$, the solution to the observer's planning task, the state of the world is updated, and $O$ is updated with any outcomes of sensing actions that were observed during the execution of $\tau$, as well as world-altering actions that belong to $\tau$\eat{ as the last observation in the sequence}. We assume $\tau$ remains applicable throughout its execution and will address the ramifications of an ever-changing world (that may render $\tau$ irrelevant) in future work. 



Algorithm 1 presents an active goal recognition algorithm which returns a set of goals $\hyps'$ $\subseteq$ $\hyps$ given an active goal recognition problem $\activeGRtuple$. We assume that at first $O$ is empty.
%
% The algorithm
% runs continually and is triggered when a new observation $O_{m+1}$ is available (Line 1). For every new observation, 
%
In Line 3, the observer's planning task is constructed as previously discussed in this section and subsequently solved, yielding $\tau$.
%
Throughout the execution of $\tau$ in Line 4, $O$ is updated with any outcomes of sensing actions that were observed during the execution of $\tau$, as well as world-altering actions in $\tau$. We assume $\tau$ remains applicable throughout its execution and will address the ramifications of an ever-changing world (that may render $\tau$ irrelevant) in future work.
%
In Line 5, we make use of a goal recognition algorithm that is assumed to take as input a goal recognition problem $\goalrectuple$ and return the optimal goal set $\optimalhyps \subseteq \hyps$. Finally, if $|\hyps'| = 1$ or some termination condition is met (e.g., timeout), the algorithm returns $\hyps'$, and repeats lines 3-5 otherwise.






% As $\tau$ is executed (Line 5), the state of the world is updated, hypotheses are (possibly) eliminated from $\hyps'$, and each test outcome that was observed during the execution of $\tau$ is appended to $O$ as the last observation in the sequence.

% The algorithm first makes use of a goal recognition algorithm (possibly one that is optimized for online goal recognition (e.g., \cite{vered2018towards}) that is assumed to take as input a goal recognition problem $\goalrectuple$ and return the optimal goal set $\optimalhyps \subseteq \hyps$\eat{ subset\commentms{return optimal goal set}*** of $\hyps' \subseteq \hyps$ which does not include eliminated hypotheses that do not conform with $O$} (Line 3).
% \eat{We assume that the goal recognition algorithm uses identical elimination criteria as those defined in the previous section. **The elimination criteria could be changed and thus different goal recognition techniques could be used.**
% The elimination criteria of the goal recognition algorithm are known to Algorithm 1 and used for plan generation (e.g., hypotheses whose optimal plans do not align with $O$ are eliminated).\commentms{define alignment? satisfaction?}}
% %

% %
% The algorithm runs continually and repeats Lines 3-5 whenever a new observation $O_{m+1}$ is available (Line 6). Finally, if $|\hyps'| > 1$ the algorithm repeats lines 2-4 and returns $a$  some termination condition is met (e.g., timeout), the algorithm returns the final set of non-eliminated hypotheses $\hyps'$ in Line 7.


\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\begin{algorithm}[h!]
\begin{small}
\floatname{algorithm}{Algorithm 1}
\renewcommand{\thealgorithm}{}
\caption{}
\label{fig:algorithm_APR}
\begin{algorithmic}[1]

\Require An active goal recognition problem
\Statex $\mathcal{P} = \activeGRtuple$, where $O$ is empty
%\linebreak
\Ensure $\hyps' \subseteq \hyps$
\State $\hyps' \gets \hyps$
\Do
\State  $\tau$ $\gets$ \textsc{GenerateObserverPlan($\mathcal{P}$)}
    \State \textsc{ExecuteObserverPlan($\tau$)}
\State $\hyps'$ $\gets$ \textsc{RecognizeGoal($\langle \Sigma_A, \init_A, \hyps', O \rangle$)}
    % \WHILE{\textbf{not} (\textsc{CheckEndingCriteria}($\hyps$) \\\textbf{or} \textit{\textsc{isAvailable}($o_{t+2} \in O$)} \textbf{or} \textit{timeout})}
    % \State \textsc{UpdateObservations($O$)}
    %\STATE $\hyps'$ = \textsc{PRAlgorithm($O,\hyps$)}
    % \ENDWHILE{}
% \ENDWHILE{}
\doWhile{$|\hyps'| > 1$}
% \WHILE{\textit{\textsc{isAvailable}($o_{m+1}$)}}
    

\State RETURN $\hyps'$




\end{algorithmic}
\label{alg1}
\end{small}
\end{algorithm} 



\begin{thm}\label{alg_1_thm} 
Given an active goal recognition problem $\activeGRtuple$ where $O$ has been updated following Line 4 of Algorithm 1, if the observer is non-intervening it follows that, following Line 5 of Algorithm 1, for each $G \in \hyps'$ there exists a $\pi \in \Pi^*(G)$ and $\pi$ \textit{satisfies} $O$.
\end{thm}

The proof is based on the fact that the goal recognition algorithm returns the optimal goal set $\hyps^{*}$ where each goal $G \in \hyps^{*}$ is compatible with observations in $O$ comprising the actor's behavior, the actions of the observer, and outcomes of sensing actions performed by the observer. Since the observer is non-intervening, if \textit{achievable($\Sigma_A$,$G$)} (resp. \textit{$\lnot$achievable($\Sigma_A$,$G$)}) holds in $b'$ for $\init'$ for some $G$ $\in$ $\hyps$\eat{(i.e., $G$ $\not\in$ $\hyps'$)}, \textit{achievable($\Sigma_A$,$G$)} (resp. \textit{$\lnot$achievable($\Sigma_A$,$G$)}) holds throughout the execution of $\tau$ and $\hyps'$ is thus not affected. 


% \subsubsection{Proof Sketch}  Let $b$ be a belief state that may result from executions advised by $\tau$ generated in Line 2 as a solution to $\langle \fluents', \actions', \sensingactions', \init', G_O \rangle$. From the construction of the planning task it follows that $G_O$ either holds or does not hold in $b$ (as $\tau$ is a weak plan). 
% %
%  then $O$ is updated with an outcome of a sensing action 
 
% Let $\hyps'$ be the output of the goal recognition algorithm called in Line 4 of Algorithm 1. $\hyps'$ is the set of goals compatible 
% If $G_O$ does not hold in $b$ then the outcome of the sensing actions added to $O$ will 

% If $G_O$ does not hold in $b$ then $\hyps'$ is left unchanged (when executing $\tau$ in Line 5), and thus $\hyps' = \hyps^{*} \subseteq \hyps$.
% If $G_O$ holds in $b$ then either some hypotheses have been eliminated or $\hyps'$ is left unchanged and thus $\hyps' \subseteq \hyps^{*} \subseteq \hyps$. Since the observer is non-intervening, if \textit{$\lnot$achievable($\Sigma_A$,$G$)} holds in $b'$ for $\init'$ for some $G$ $\in$ $\hyps$ (i.e., $G$ $\not\in$ $\hyps'$), \textit{$\lnot$achievable($\Sigma_A$,$G$)} holds throughout the execution of $\tau$ and $\hyps'$ is thus not affected.  \hfill $\blacksquare$





\eat{returns  if the observer is non-intervening.}
% \eat{ and (2) if $\hyps''$ is the set of hypotheses returned by Algorithm 1 without executing Lines 3-4 then $\hyps' \subseteq  \hyps''$.}
% \eat{
% Let $\hyps^{PR}$ be the result of executing Line 2 of Algorithm 1 once. Then, assuming the goal recognition algorithm used in Line 2 is correct it follows that\\

% \eat{\commentms{we maybe want $\hyps' \subseteq \hyps$ per the spec or just prove that $G^* \in \hyps'$}}}
% % =====================
% % Correctness of algorithm relative to the different approaches
% % E.g., if test is relevant, then H necessarily decreases in size. \textbf{Show that theorem 1 is fulfilled by lm approach since if we manage to elimiante all but one hypothesis then only G*is left}. 
% % \commentms{if the goal recognition algorithm and planner used are correct - wrt their respective specifications - i.e., goal rec alg returns $\hyps^{*}$ given input and planner returns $\tau$ that solves planning task (be it a weak, strong, or strong cyclic) plan}

% % \commentms{proof is that goal rec alg returns the optimal goal set and steps 4-5 either add outcomes of sensing actions to $O$ such that the optimal goal set is changed or not changed.}


% %NOTE
% % it may be the case that the most unique landmarks are shared by ALL hyps in $\hyps'$. In that case, both a a positive and a negative outcome in $\tau$ will NOT eliminate any hypotheses in $\hyps'$

% % \textbf{MODIFY PROOF to FIT NEW OUTPUT OF ALG - show that we get $\optimalhyps$ after line 3 (assuming correctness of gr alg which we assume in theorem) and that lines 4 and 5 either return $\optimalhyps$ or subset of that}

% % \subsubsection{Proof Sketch} Let $s$ be a state that may result from the execution of the action tree generated in Line 4 as a solution to $\langle \fluents', \actions', \sensingactions', \mathcal{I}_O, G_O', \statecons \rangle$. From the construction of the planning task it follows that $\textit{testsExhausted}$ $\lor$ $G_O$ (but not both) holds in $s$.
% % \eat{In Line 5, at the end of the execution path of the action tree generated by the planner either \textit{testsExhausted} or \textit{eliminated} will be satisfied.}
% % If \textit{testsExhausted} holds in $s$, then all test outcomes have been negative, $\hyps'$ is left unchanged, and thus $\hyps' \subseteq \hyps$.
% %
% % and thus in Line 6 $O$ is not updated with new observations. Thus, in Line 7, the PR algorithm will return the same result returned by the algorithm in Line 2, i.e., $\hyps^{PR}$.
% %
% % If $G_O$ holds in $s$ then all hypotheses but one are eliminated and $|\hyps'| = 1$ and thus $\hyps' \subseteq \hyps$. $\blacksquare$
% % $O$ is updated with one of the positive test outcomes ****and the PR algorithm will eliminate all hypotheses but one, since its elimination criteria match those of our approach\commentms{do we want to do elimination instead of the PR alg?}***. Following Theorem 1, since $|\hyps| = 1$ we have that $\hyps' = \{G^{*}\}$.



% % \begin{corro}\label{thm_correct}
% % Let $\hyps'$ and $\hyps''$ be the sets of hypotheses returned by Algorithm 1 and Algorithm 1 without Lines 3-4. It then follows that $\hyps' \subseteq  \hyps''$.
% % \eat{Let $\hyps^{PR}$ be the result of executing Line 2 of Algorithm 1 once. Then, assuming the goal recognition algorithm used in Line 2 is correct it follows that following the execution of Lines 3-4 of Algorithm 1, $\hyps' = \hyps^{PR}$ or $\hyps' \subseteq \{G^{*}\}$.} \commentms{need assumption about $\statecons$ and GR alg? maybe add as (2) to theorem 1 - NO NEED FOR CORROLOARY (which is curerntly false) if we prove that we get $\hyps' \subseteq \hyps^*$}
% % \end{corro}

% % Thus, the observer's actions may eliminate hypotheses in $\hyps$ that would not otherwise be eliminated were the observer to passively await new observations.

% % \begin{thm}\label{thm_correct}
% % Algorithm 1 returns a subset of the hypotheses $\hyps' \subseteq \hyps$.\commentms{only prove this ONE!}
% % \end{thm}

% % Theorem \ref{thm_correct} follows from Theorem \ref{alg_1_thm}.


% % \commentms{test generation process induces a conditional/contingent planning problem}



% Next, assuming an optimal planner:

% The planning task in generated in Line 4 contains an incomplete initial state as well as sensing actions. Thus, assuming $\Omega \neq \emptyset$, the planning task is a conditional/contingent planning problem and thus Theorem \ref{thm:complexity} follows 


% \begin{thm}
% Let $\hyps'$ and $\hyps''$ be the sets of hypotheses returned by Algorithm 1 and Algorithm 1 without Lines 3-4. Then it follows that $\hyps' \subseteq  \hyps''$.
% \end{thm}


% \begin{thm}[Minimality of Tests] Landmark-based elimination tests are minimal (Definition \ref{minTest}).
% \end{thm}

% Follows from the correspondence between test generation and planning. There isn't another way to eliminate all hyps (that we know of) and we found The minimal test.thus, it's The minimal test to eliminate between all hypotheses.are we proving minimality of the complex test? There's no other n-1 eliminating test with less steps in each Branch of tree

% Test outcomes can also confirm a hypothesis. For example, let us assume OBS cannot see what ACT has placed on the counter, and has only observed that ACT has turned on the kettle. OBS can perform a test which includes walking to the kitchen counter and stove and sensing what is on it. THERE'S  A POT IN THE ORIGINAL EXAMPLE. NOW THERE"S NOT. If the test outcome is \textit{on(pot,stove))} then this confirms both RICE and PASTA but does not confirm TEA, thus eliminating it. \textbf{Hypothesis confirmation is tricky with noise (e.g., the pot was left on the stove yesterday and never removed) }. But so is PR\\

% % Recall the DPR task in which we would like to disambiguate the hypotheses. 
% We can now make use of landmarks in order to translate the DISCRIMINATE/disambiguation epistemic goals to goals that can be given to a planning system (???). For example, consider the epistemic goal DISCRIMInATE(PASTA,RICE). To discriminate between the two hypotheses, we can refute one or the other. Thus, DISCRIMInATE(PASTA,RICE) $=$\commentms{what symbol should be here?} $K_{\textsc{Obs}}$ \textit{eliminated(RICE)} OR $K_{\textsc{Obs}}$ \textit{eliminated(PASTA)}, where a hypothesis can be eliminated as described above, either by being refuted or by not being confirmed. Thus, we can translate  $K_{\textsc{Obs}}$ \textit{eliminated(RICE)} $\lor$ $K_{\textsc{Obs}}$ \textit{eliminated(PASTA)}, using their landmarks, to $K_{\textsc{Obs}}$\textit{$\lnot$(in(rice,cabinet) $\land$ $\lnot$on(rice,counter)) $\lor$ ($\lnot$in(rice,cabinet) $\land$ on(rice,counter))} $\lor$ $K_{\textsc{Obs}}$\textit{$\lnot$(in(pasta,cabinet) $\land$ $\lnot$on(pasta,counter)) $\lor$ ($\lnot$in(pasta,cabinet) $\land$ on(pasta,counter))}. Since $K_{\textsc{Obs}}$\textit{$\lnot$on(rice,counter) $\land$ $\lnot$on(pasta,counter)}, the above simplifies to $K_{\textsc{Obs}}$\textit{$\lnot$in(rice,cabinet)} $\lor$ $K_{\textsc{Obs}}$ \textit{$\lnot$in(pasta,cabinet)}.
% \\ \commentms{can any of these be converted to KnowWhether??}
% \textbf{Formal translation of elimination (or even discrimination) goals to landmark-based epistemic goals}
% Discrimination goal is translated to a bunch of disjunctive clauses - one could be using consistency based and one using abductive space (e.g., (not (in (pasta cabinet))) OR (on milk counter)

% Recall that an abductive hypothesis is eliminated if it is not confirmed by $\testoutcome$. We acknowledge that this definition of elimination may not always be appropriate in the PR case. For example, this definition does not allow for any (what would be perceived as) sub-optimal behavior (relative to \act's model)  as such behavior would eliminate any hypotheses, even if the agent is in fact following the hypothesis. However, this definition of elimination holds under the assumption that \act is following optimal paths to the goal (wrt \act's model of the world). We posit that this assumption holds in various domains of interest. For instance, in a time-sensitive setting (e.g., care giving or search\&rescue) it is reasonable to assume that an agent will follow optimal paths to the goal. Thus, if an agent is observed to perform an action that does not serve a certain goal, that goal can fairly confidently be eliminated as a possible hypothesis to explain the observations. It is therefore reasonable to eliminate a hypothesis $h$ if we observe a landmark $l$ that can only become true from some action's effect, and $l$ is not a landmark for $h$.

%\subsubsection{LTL pattern-based Hypothesis Elimination}



% \subsection{Multiple Goals}
% For multiple goals, if we refute any one of the landmarks in the conjunction of the sets of landmarks for both goals, then both, together, are not possible


% \subsection{Epistemic Landmarks}
% We observe that ACT went to point A and then \textbf{we lose track of ACT} - thus, we can’t discriminate between the hyps (at ACT base) and (at ACT B). We know goal is ‘find a victim and report to base or return to base if no victims found' \textbf{in a way, this is plan recognition. we know abstract goal and we can't discriminate between PLANS}\\
% \textbf{How do we figure out that the test is finding out whether there's a victim at point A}
% \begin{itemize}
%     \item when computing landmarks for (at ACT base) from the current initial state, we know that ACT will only go to base (report) if it has finished surveying all points or knows that there is an individual at A (or knows that there is an individual at B …) - so landmarks will be K\_ACT(at victim A). so OBS can go to A and find out whether (at victim A) holds (OBS can already infer that ACT kWhether (at victim A) because of the observations (axiom) \textbf{what's the initial state from which we compute landmarks? maybe just $K_{ACT}(at victim A)$ is enough}
%     \begin{itemize}
%         \item knowing that ACT knows that there’s a victim at A will refute the hyp (at ACT B) since the landmark for that is K\_ACT(not (at victim A)) THIS RELATES to notion of ADEQUACY
%     \end{itemize}
% \end{itemize}

% \textbf{It doesn't matter if there's neither tea nor coffee.} Act might still be intending to make one of them. If we find neither, then we still don't know what ACT intends to do. it also doesn't matter - because we know that goal is not possible and can let ACT know. If we refute all hypotheses, then we should reason that either our hypotheses are wrong/model of ACT is wrong/ACT has false beliefs. Next thing to do is do assume (or find out which one it is and then reason what's wrong about it - for example, we can reason that ACT has false beliefs pertaining to contents of cabinet if we assume our model is correct (maybe ACT can make something else for dinner and we DO Not kNOW THIS))\textbf{future work??}


% \textbf{possible theorem: }our translation from DISCRIMINATE to ELIMINATE to epistemic goal using landmarks is sound and complete (in that hyps are really discriminated) given certain assumptions(?)





% \section{AI Planning-based Diagnostic Plan Recognition (or AI planning based test generation OR DPR as (Epistemic) Planning) OR Computing Diagnostic Plans} \label{comp}


% Given a DPR task, \commentms{define DPR tuple macro}, we wish to return a subset of the hypotheses. To do so, we eliminate hypotheses using the landmark-based approach discussed in the previous section. Can we therefore translate the hypotheses disambiguation goal to an epistemic goal such as $K_{\textsc{Obs}}$\textit{$\lnot$in(rice,cabinet)} $\lor$ $K_{\textsc{Obs}}$ \textit{$\lnot$in(pasta,cabinet)} in our example. To achieve an epistemic goal, we require a planning system that can reason over knowledge states. \textit{The notion of planning and reasoning to achieve a state of knowledge dates back to work by Moore (1985). Scherl and Levesque (2003) later integrated Moore’s approach with Reiter’s solution to the frame problem (1991). More recently, epistemic planning has been discussed in the context of dynamic epistemic logic (e.g, (Herzig, Lang, and Marquis 2003; Andersen, Bolander, and Jensen 2012).} \commentms{discuss epistemic planning advancements}.\\

% We make use of epistemic planners to automatically generate tests that can eliminate the hypotheses. These tests (e.g., sensing the contents of the kitchen cabinet) may require both world altering actions as well as sensing, purely epistemic actions which only change the agent's state of knowledge. Thus, we require a planning system that can handle non-deterministic sensing actions and epistemic goals. Then, the goal $K_{\textsc{Obs}}$\textit{$\lnot$in(rice,cabinet)} $\lor$ $K_{\textsc{Obs}}$ \textit{$\lnot$in(pasta,cabinet)} $\lor$ $K_{\textsc{Obs}}$ \textit{in(pasta,cabinet) $\land$ in(rice,cabinet)}can be given directly to the planner which will automatically generate a diagnostic plan which will either eliminate either RICE or PASTA, thereby discriminating between the two hypotheses, or confirm the two hypotheses (\textbf{it's a relevant test! there are no discriminating tests for these two hypotheses}).\\

% In our example, a relevant test that can discriminate between RICE and PASTA consists of the following (assuming the agent is not close to the cabinet??): \textit{move(currLoc,cabinet);sense\_cabinet}.  \commentms{Sometimes OBS may need to change their point of view in order to see something. E.g., counter is out of view for OBS. need to move in order to see what it is - then I can see that you're holding pasta. Can use vision-knowledge work by Francois}





% \subsection{Landmark Generation}
% Talk about various landmark generation algorithms \commentms{can we easily use these on epistemic planning domain with sensing actions}






% \subsubsection*{Strategies for Hypothesis Elimination}\label{strategies_elim}
% % \subsubsection{Maximally Eliminate Equally Likely Hypotheses} 
% If there are no unique landmarks or sufficient protected landmarks, it may not be possible to eliminate all hypotheses but one. Since the recognition task is to infer the actor's goal, eliminating some hypotheses is preferable to eliminating none.
% %
% % Instead, the observer may attempt to maximally eliminate hypotheses in $\hyps^{*}$. A simple, PDDL-specific approach to facilitate maximal elimination includes defining a function which counts the number of eliminated hypotheses. The planner's goal is then to maximize the value of this function by finding a maximally eliminating conditional plan. Alternatively, a set of maximally eliminating landmarks could be generated 
% %
% % What should we do when we cannot eliminate all hypotheses but one? Since our task is to infer the actor's goal, eliminating some hypotheses is preferable to eliminating none. 
% %
% Thus, we can follow a simple approach to maximally eliminate hypotheses. From the set of all landmarks ($\mathcal{L})$, we find a subset of landmarks $\mathcal{L}_{max\_elim}$ with the highest `uniqueness value' \cite{pereira2017landmark}.
% %
% % such that the number of hypotheses associated with each $l \in \mathcal{L}_{max\_elim}$ is minimal \commentms{this can be formalized}. 
% %
% For instance, we may find that there are no unique landmarks in $\mathcal{L}$ but only landmarks that are associated with two hypotheses. Thus, a test outcome $\testoutcome$ which is a landmark in $\mathcal{L}_{max\_elim}$ will eliminate all hypotheses but those it is associated with. We augment $\mathcal{A}$ similarly to before with actions whose preconditions include landmarks from $\mathcal{L}_{max\_elim}$ and \textit{eliminated} as the effect. We similarly treat the set of protected landmarks in an attempt to find the maximally eliminating tests. 

% The above can be construed as a simple information-theoretic approach wherein we attempt to reduce our uncertainty about $\hyps$ when the hypotheses are assumed equally likely. If the hypotheses in $\hyps$ are associated with probabilities, a possible approach would be to only focus on the most likely hypotheses that will maximize information gain wrt $\hyps$. A heuristic which guides the elimination efforts may be desirable in general to minimize valuable testing time on improbable hypotheses. \commentms{mention SPR techniques?}

% as the computational cost of discriminating between all hypotheses may be too large}.\\

% Thus, the planning goal constructed in Line 4 the maximum number of hypotheses that can be eliminated.

% , initially, the ending criterion is $|\hyps
% | = 1$ and thus we first attempt to eliminate all hypotheses but one. If \textit{testsExhausted} is satisfied by the action tree (i.e., no hypotheses are eliminated) we set the ending criterion to $\mathcal$


% randomly choose $|\hyps'| - 1$ hypotheses and 
% first generate a goal for DISCRIMINATE\_ALL\_HYPS. If this fails, for all permutations (???) of $n-1$ hypotheses out of the $n$ hypotheses in $H$, attempt to generate a plan for DISCRIMINATE\_N-1\_HYPS.

% the ending criteria of the APR algorithm is $|H| = 1$ (OR UNTIL IT IS no longer possible to eliminate!). To this end, we must discriminate between all hypotheses in $H$. That is, we must eliminate all but one hypothesis in $H$. Sometimes, we may not be so lucky as to have a test (possibly) eliminate all hypotheses but one as seen in our kitchen example. For example, given $H = h1, h2, h3$ the `best' we can do might be to eliminate one hypothesis, leaving two `standing'. Since our task overarching objective is to disambiguate the set of hypotheses, eliminating one hypothesis is preferable to eliminating zero. How, then, are we to select which hypotheses should be eliminated if we cannot eliminate all hypotheses? Many approaches have been proposed in the past to select a ... \commentms{from SPR}. 

% \subsubsection{Information-theoretic Approaches}
% For example, if probabilities are associated with the hypotheses then our strategy could be to try to discriminate between the most likely hypotheses \commentms{this might also be desirable in general, as the computational cost of discriminating between all hypotheses may be too large}.\\

% Assuming all hypotheses are equally likely (as in kitchen example), we can employ the following simple strategy: \commentms{NEED TO FORMALIZE THIS with goals and DISCRIMinATE}attempt to generate a diagnostic plan for DISCRIMINATE\_ALL\_HYPS. If this fails, for all permutations (???) of $n-1$ hypotheses out of the $n$ hypotheses in $H$, attempt to generate a plan for DISCRIMINATE\_N-1\_HYPS.

==> sections/discussion_and_summary.tex <==
\section{Discussion and Summary}\label{sec:disc_sum}



In this work, we have introduced and formalized the notion of active goal recognition, where we endow the observer with agency to act in the world in order to expedite (and in some cases make possible) the recognition of the actor's goal. We presented an algorithm for active goal recognition and a landmark-based approach that leverage automated planning to facilitate hypothesis elimination. Finally, we evaluated our approach on a diversity of domains and demonstrated the merits of an active observer, including earlier recognition compared to a passive observer.

% There is a diverse body of research related to the ideas we have presented. 
%
As mentioned in Section \ref{intro}, our work is situated within the broader field of plan, activity, and intent recognition. Most closely related to our work is a body of work on plan and goal recognition that endows the observer with agency to act in the world (and possibly interact with the actor) in order to disambiguate the hypothesis space \textit{during runtime} (e.g., \cite{bisson2011provoking,fagundes2014dealing,mirsky2016sequential}). While \citeauthor{kabanza2010opponent} (\citeyear{kabanza2010opponent}) independently propose to allow the observing agent to actively make observations (e.g., sending scouts to enemy territory), they use plan libraries and, to the best of our knowledge, have not implemented their approach. In the \textit{offline} setting, the body of work on goal recognition design can also be seen to endow the observer with agency to modify the environment \cite{keren2014goal} or to provide the actor with information \cite{2019InformationSF} to benefit hypothesis elimination during the eventual runtime. In all of these works, the observer selects tests whose outcomes (e.g., the actor's next action or response to a query) facilitate hypothesis elimination and are therefore important modalities at the avail of an active observer.

% The agency afforded to the observer in these works (e.g., modifying the environment, `provoking' the actor or providing the latter with information) place the observer at different points along an `intervention continuum' and 

% rver in these works (e.g., modifying the environment, `provoking' the actor or providing the latter with information) place the observer at different points along an `intervention continuum' and are important modalities at the avail of an active observer

% (controlled by $\statecons$) can therefore be seen as various modalities available to an active observer.


Another related body of work that equips the observer with agency focuses on the observer's \textit{reaction} to the inferred goal rather than on hypothesis disambiguation.
%
% Previous work has also explored one aspect of an active observer, where planning and recognition are integrated.
%
\citeauthor{freedman2017integration} (\citeyear{freedman2017integration}) show how the observer can be made to aid, impede, or not interfere with the actor, while work on counterplanning (e.g., \cite{pozanco2018counterplanning}) enables an observer to devise a counterplan which aims to impede goal achievement.

% via appropriate constraining of a joint observer-actor planning task. 
% %
% \eat{The authors also 
% may assist the actor by adopting its goal or hinder the actor by preventing it from achieving its goal \commentms{Freedman also enforce constraints on the behavior of the observer, forcing it to either intervene (assistive and adversarial) or not interfere (independent interaction)}.}
% %
% Further, work on counterplanning (e.g., \cite{pozanco2018counterplanning,porteous2019protagonist}) show how an observer can devise a counterplan which aims to impede goal achievement.
% prevent the actor from achieving its goal. 

% While these works share our motivation and imbue the observer with agency, they do not explore ways in which the observer may act in the world to hasten the recognition process. Our work therefore complements this body of work.

% toolbox.


% The common thread running through these works is the observer


% \citeauthor{mirsky2016sequential} (2016) introduce the sequential 
% process for reducing the
% set of possible hypotheses called Sequential Plan Recognition (SPR). SPR iteratively queries
% the user and revises the set of possible hypotheses according to the outcome of the query.

% Hypothesis Elimination and disambiguation in GR/PR
% and Testing the Actor’s Response Take Hypothesis disambiguation in plan recognition section from SPR paper
% Both GRD work (including information shaping) and provocation work have shown that by acting in and changing the
% state of the world (or ACT ’s mental state), the actor’s next
% action (response to the change in the world or mental state)
% can help disambiguate G by only confirming certain hypotheses. SPR also tests the ACT ’s response by querying
% it and eliminating hypotheses based on the response. GRD
% work (?) introduce the notion of wcd and how to modify
% D in order to minimize the wcd value. For example, by re- 
% ducing the wcd to 1, we only need to observe the actor’s next action in order to discriminate between the various hypotheses. Thus, we can generate a test in the following way: first, compute the wcd for every G ∈ G as described (?) (using current init state, with the observations compiled away). Then, we use algorithms proposed by (?) to find modifications that reduce wcd to 1. Our test then comprises of the test’s initial conditions, which involves modifying the environment (or providing the actor with information), followed by the test itself, which involves sensing the actor’s next action. The test outcome will then eliminate all but one hypohteses (in the case of wcd = 1). Eliminated is translated via wcd computation to (sensed act action) goal where the initial conditions for sense act action test is that we told act something. it doesn’t matter what action we observe since the next action will eliminate all but one hyp (what if we can only get wcd of 2 or 3 or...). Keren et al. basically modify the domain such that unique landmarks emerge for each hypothesis.

% Goal recognition is situated within the broader problem of plan, activity, and intent recognition whose various sub-problems are concerned, together, with inferring not only the actor's `top-level' goal, but also the plan that achieves this goal (where the plan being carried out by the actor is possibly independent of a specific final goal), and even the `low-level' actions, or activities of the actor \cite{sukthankar2014plan}. While approaches to goal (and plan) recognition have often matched between the observed behavior of the actor and pre-defined plan libraries (e.g., \cite{kautz1987formal,geib2009probabilistic}), the past decade has seen the rise of plan and recognition approaches that utilize planning domains (e.g., \cite{RamirezG09,sohrabi2016plan,pereira2017landmark}). Further, 
% a body of previous work has identified that performing the recognition \textit{online}, while the actor's plan is still being carried out, is  critical and has thus proposed efficient and optimized approaches geared towards online recognition (e.g., \cite{bui2003general,vered2018towards}).





% we have communicative actions with the told(x) effect. show in Sarah's partially observable wumpus domain that we cannot discriminate after first obs. The only thing to do is to tell agent something which will guarantee disambiguation in x steps. compute wcd for each test? formulate the problem as a grd problem with knowledge? Part of disjunctive goal is told(OBS, ACT, fact) where if act knows fact then by observing act's next action we will be able to discriminate between hyps. Tell action could have high cost. Similarly, we could change something physically. we can also use PR design!\commentms{perhaps this paragraph should go in discussion section - SPR also sort of goes here as we are testing the user's response to query}.

%  Bisson et al. [9] suggest to “provoke” the acting agent to perform an action that will disambiguate between two possible goals. (from SPR related work) \textbf{THEY ALSO VIEW the OBSEVER"S decision making as a planning task!!} in \cite{kabanza2010opponent}, they independently propose the notion of allowing the observing agent to act in the world in order to actively make observations (e.g., sending scouts to enemy territory in a real-time strategy game). However, they use plan libraries and, to the best of our knowledge, have not implemented their approach. Kabanza use plan libraries and haven't formalized active observations\commentms{VERIFY!}. Accordingly, our goal recognition algorithm takes as input two thresholds, one for the minimal entropy and the other for the minimal expected disambiguation. If both thresholds are met, the provocation of the event is given as a goal to a deterministic forward-chaining planner to produce a plan leading to a state where the event holds \commentms{this is what I had in mind for WCD computation in `online' GRD}
 
 
% Counterplanning using Goal Recognition and Landmarks - they analyze the planning task and look for \textbf{unachievable landmarks} that can be made true (their negation is made true) by a counterplan - thus rendering the goal unachievable. However, they don't show how to use this to hasten recogntion. Our approach can complement theirs. they say that \textit{``performance depends on the ability of the preventing agent to quickly infer
% the hidden goal, and the number of landmarks of the seeker’s
% planning task."} \textit{we rather
% explore a heuristic approach that consists in selecting the
% event to provoke just based on its expected disambiguation of the current set of hypotheses. For each provokable event, we compute the expected reduction of the uncertainty on the opponent’s intentions, knowing how he would react to the provocation. We use entropy as a measure of uncertainty associated with the set of hypotheses, and determine the provokable event that is expected to reduce it the most}



Our work is also situated within the field of human-aware AI (and planning more specifically), interested in generating agent behavior that is interpretable to the human (cast as the observer) in the loop. Recently, there has been notable interest in this field, evident by a large body of work with applications to human-human, human-machine, and machine-machine interaction. 
%
% ranging from legibility - human-human human-robot - (e.g., \cite{aksljdklas;asdkljaksd}), to obfuscation (e.g., \cite{klasjdk}), to foo-bar (e.g., \cite{akljd}).
%
% Recently, the field of human-aware AI and planning more specifically \commentms{and explicable etc.} has seen an exciting and impressive growth (in interest?), evident by a large body of work ranging from legibility - human-human human-robot - (e.g., \cite{aksljdklas;asdkljaksd}), to obfuscation (e.g., \cite{klasjdk}), to foo-bar (e.g., \cite{akljd}). \citeauthor{chakraborti2019explicability} (\citeyear{chakraborti2019explicability})
%
\citeauthor{chakraborti2019explicability} (\citeyear{chakraborti2019explicability}) present a comprehensive survey of this landscape, as well as independently discuss the notion of an active observer and how the observer's agency should affect the decision making of an actor keen on obfuscating its plan or making it more legible. \eat{Our work falls within that scope and }The ideas we have formalized in this work can be leveraged to facilitate an active observer in this context. Specifically, our work could be extended to address an actor that is assumed to be attempting to obfuscate its plan or make it more legible, as is typically the case in the aforementioned body of work. 

% Future work will also address settings where the actor may be partially informed or harbor false beliefs.

% , as is the case in the aforementioned body of work.


% it would be interesting to explore how an active observer should reason given an actor that is assumed to be attempting to obfuscate its plan or make it more legible, as is the case in the aforementioned body of work.

% since the actor in the aforementioned body of work is assumed to be attempting to make its its plans known (or obfuscated), 
%
% of foo-bar planning/human-aware planning. 
%
% While in this work we operate within a \textit{keyhole} recognition setting \cite{perraultETAL} where the actor is assumed to **not be aware of the observer\commentms{take phrsing from perrault et al}**, while in the aforementioned body of work on legibility and obfuscation, the actor is assumed to be trying to make its plans known (or obfuscated), which is the \textit{intended} recognition setting \cite{perrault}. It would be interesting to explore this setting. it would be interesting to explore both this case and where the actor is adversarial and trying to obfuscate (we see that we can partially deal with this case in the intrusion detection)


% Finally, exciting avenues for future research abound. 
%
\eat{Our approach to hypothesis elimination can be construed as a simple information-theoretic approach wherein we attempt to reduce our uncertainty about $\mathcal{G}$ when the hypotheses are assumed equally likely.}
%
Finally, if probabilities are associated with hypotheses in $\hyps$, the observer can focus on hypotheses that will maximize information gain wrt $\hyps$. A heuristic which guides the elimination efforts may be desirable in general to minimize valuable testing time on improbable hypotheses, as shown by \citeauthor{mirsky2016sequential} (\citeyear{mirsky2016sequential}) who employ information-theoretic strategies to determine how to best query the actor. Importantly, there is often no need to eliminate all hypotheses. E.g., in the \textsc{Terrorist} domain, in order to plan a reaction, it suffices to discriminate between two sets of hypotheses (e.g., is the actor heading east or west). 

% Finally, we assume in our experimentation that the actor has a classical planning task and we want to address an actor with partially observable

% For instance, in order to prevent the agent from achieving its goal, it may suffice to discriminate between G1 and G2 or between G1 and G3, while not caring about discriminating between G2 and G3.

% \begin{itemize}
%     \item information-theoretic strategies for hyp elim
%     \begin{itemize}
%         \item 
%         \item \citeauthor{sohrabi2016plan} (\citeyear{sohrabi2016plan}) treat noisy and missing observations ***and we will address this case in the future.***
%     \end{itemize}
% \end{itemize}

% \begin{itemize}
%     \item what if \act has false beliefs?
%     \item what if actor changes its goal/plan or has multiple goals
% \end{itemize}





% \subsubsection*{Acknowledgments} 

% The authors gratefully acknowledge funding from NSERC and thank their colleague Toryn Q. Klassen for helpful discussions.


% \break
